Large-Scale Dynamic Predictive Regressions

We develop a novel "decouple-recouple" dynamic predictive strategy and contribute to the literature on forecasting and economic decision making in a data-rich environment. Under this framework, clusters of predictors generate different latent states in the form of predictive densities that are later synthesized within an implied time-varying latent factor model. As a result, the latent inter-dependencies across predictive densities and biases are sequentially learned and corrected. Unlike sparse modeling and variable selection procedures, we do not assume a priori that there is a given subset of active predictors, which characterize the predictive density of a quantity of interest. We test our procedure by investigating the predictive content of a large set of financial ratios and macroeconomic variables on both the equity premium across different industries and the inflation rate in the U.S., two contexts of topical interest in finance and macroeconomics. We find that our predictive synthesis framework generates both statistically and economically significant out-of-sample benefits while maintaining interpretability of the forecasting variables. In addition, the main empirical results highlight that our proposed framework outperforms both LASSO-type shrinkage regressions, factor based dimension reduction, sequential variable selection, and equal-weighted linear pooling methodologies.

==> Tables/Old/Table001.tex <==
% Table generated by Excel2LaTeX from sheet 'Regression'
\begin{sidewaystable}[htbp]
\caption{Statistical Comparison of Models Combination Schemes: Stock Returns Predictability}
\vspace{.1in}
\begin{justify}
\footnotesize{This table reports an out-of-sample comparison of our predictive framework against standard model combination methodologies, across ten different industries. Performance comparison is based on the Root Mean Squared Error (RMSE), and the Log Predictive Density Ratio (LPDR) as in Equation \eqref{eq:lpdr}. We report the results obtained for each of the group-specific predictors, the results obtained by simply taking the historical average of the stock returns (HA), and the results from a set of competing model combination/shrinkage schemes, e.g. LASSO, Equal Weight, and Bayesian Model Averaging (BMA). Following \cite{McAlinn2017} we label our modeling framework Bayesian Predictive Synthesis (BPS). The sample period is 01:1970-12:2015, monthly.}
\end{justify}
\renewcommand{\arraystretch}{1.2}
\vspace{1em}
{\bf Panel A: \normalfont Root Mean Squared Error} \vspace{0.2cm}\\ 		
\resizebox{1.1\textwidth}{!}{\begin{tabular}{lcccccccccccccccc}
\hline
Industry & \multicolumn{10}{c}{Group-Specific Models}                                                                 & HA    & Full & LASSO & Equal Weight & BMA & BPS \\
\cline{2-11}
         & Value	&Profit	 & Capital	& Soundness	 &Solvency	&Liquidity	&Efficiency	&Other	&Aggregate Fin	&Macro  &\\
\hline
Durbl    & 0.102	&0.103	 &0.085	    &0.103	     &0.089	    &0.086	    &0.089	    &0.084	&0.086	        &0.095  & 0.079 &0.484 & 0.091 & 0.084 & 0.084	& 0.078\\
NoDurbl  & 0.044	&0.043	 &0.038	    &0.046	     &0.038	    &0.036	    &0.040	    &0.038	&0.041	        &0.042  &0.034  &0.162 &0.038  & 0.036 & 0.036	&0.034\\
Manuf    & 0.064	&0.072	&0.055	&0.077	&0.057	&0.057	&0.058	&0.054	&0.058	&0.061 &0.052 &0.338	&0.056	&0.054	&0.054	&0.052\\
Energy   & 0.069	&0.086	&0.062	&0.082	&0.064	&0.061	&0.067	&0.061	&0.066	&0.070 & 0.060 & 0.511	&0.062	&0.063	&0.061	&0.059\\
HiTech   & 0.078	&0.110	&0.069	&0.105	&0.076	&0.074	&0.079	&0.071	&0.078	&0.083 & 0.069 & 0.516	&0.079	&0.071	&0.070	&0.068 \\
Health   & 0.047	&0.052	&0.043	&0.057	&0.042	&0.041	&0.043	&0.041	&0.045	&0.046 & 0.040 & 0.241	&0.041	&0.042	&0.041	&0.039\\
Shops    & 0.056	&0.056	&0.047	&0.064	&0.048	&0.047	&0.049	&0.047	&0.051	&0.051 & 0.044 & 0.263	&0.047	&0.046	&0.048	&0.043\\
Telecomm & 0.068	&0.064	&0.058	&0.073	&0.058	&0.055	&0.059	&0.058	&0.057	&0.060 & 0.054 & 0.348	&0.056	&0.054	&0.058	&0.053\\
Utils    & 0.048	&0.054	&0.043	&0.072	&0.044	&0.045	&0.046	&0.041	&0.047	&0.048 & 0.041 & 0.610	&0.046	&0.042	&0.041	&0.040\\
Other    & 0.071	&0.070	&0.056	&0.084	&0.057	&0.057	&0.060	&0.056	&0.063	&0.062 & 0.054 & 0.415	&0.058	&0.056	&0.056	&0.053\\
\hline
    \end{tabular}}%
\vspace{1em}

{\bf Panel B: \normalfont Log-Predictive Density Ratio} \vspace{0.2cm}\\ 		
\resizebox{1.1\textwidth}{!}{\begin{tabular}{lcccccccccccccccc}
\hline
Industry & \multicolumn{10}{c}{Group-Specific Models}                                                                 & HA    & Full & LASSO & Equal Weight & BMA & BPS \\
\cline{2-11}
         & Value	&Profit	 & Capital	& Soundness	 &Solvency	&Liquidity	&Efficiency	&Other	&Aggregate Fin	&Macro  &\\
\hline
Durbl    & -76,59	&-91,97	&-36,33	&-93,09	  &-44,81	&-39,51	&-45,30	&-34,21	&-44,15	&-62,84 &-23,67  &-2436	  &-227,3	&-24,06	&-34,69	&-\\
NoDurbl  & -66,96	&-64,74	&-25,99	&-77,46	  &-30,96	&-17,77	&-34,80	&-23,95	&-44,61	&-49,45 &-10,12  &-1692	  &-261,3	&-15,81	&-18,74	&-\\
Manuf    & -65,68	&-88,08	&-29,68	&-132,12	&-36,36	&-34,08	&-39,40	&-23,94	&-45,47	&-51,13 &-18,62  &-2845	  &-276,8	&-14,75	&-23,00	& -\\
Energy   & -31,77	&-93,31	&-9,96	&-83,42	  &-14,61	&-5,77	&-24,30	&-6,08	&-19,92	&-32,40 &-2,83   &-2717	  &-219,6	&-8,93	  &-6,61	  &-\\
HiTech   & -47,46	&-95,81	&-20,39	&-101,32	&-28,36	&-29,41	&-40,36	&-22,14	&-37,87	&-48,17 & -16,10 & -2419	&-296,4	&-19,34	&-20,92	&-\\
Health   & -43,09	&-77,01	&-20,48	&-90,36	  &-17,71	&-12,62	&-26,84	&-12,33	&-36,88	&-40,45 & -8,09  & -2066	&-269,8	&-11,04	&-13,67	&-\\
Shops    & -59,31	&-61,68	&-19,50	&-100,51	&-24,30	&-20,11	&-26,68	&-19,07	&-36,97	&-35,68 & -8,49  & -1952	&-237,0	&-15,92	&-23,90	&-\\
Telecomm & -85,13	&-57,67	&-37,53	&-83,81	  &-37,00	&-30,89	&-43,95	&-32,30	&-38,45	&-48,80 & -22,33 & -2422	&-258,9	&-23,68	&-31,34	&-\\
Utils    & -43,13	&-66,39	&-15,49	&-146,62	&-19,73	&-24,01	&-28,36	&-12,03	&-39,62	&-44,05 & -10,98 & -5545	&-305,2	&-11,21	&-12,09	&-\\
Other    & -108,53&-89,30	&-39,48	&-150,83	&-40,52 &-38,49	&-45,34	&-38,71	&-72,47	&-58,40 & -29,26 & -3523	&-246,7	&-23,81	&-38,57	&-\\
\hline
    \end{tabular}}%
\label{Table001}

\end{sidewaystable}%


==> Tables/Old/Table002.tex <==
% Table generated by Excel2LaTeX from sheet 'Regression'
\begin{sidewaystable}[htbp]
\caption{Economic Comparison of Models Combination Schemes: Stock Returns Predictability}
\vspace{.1in}
\begin{justify}
\footnotesize{This table reports an out-of-sample comparison of our predictive framework against standard model combination methodologies, across ten different industries. Performance comparison is based on the Sharpe Ratio (SR), and its modification whereby short sales are not allowed. We report the results obtained for each of the group-specific predictors, the results obtained by simply taking the historical average of the stock returns (HA), and the results from a set of competing model combination/shrinkage schemes, e.g. LASSO, Equal Weight, and Bayesian Model Averaging (BMA). Following \cite{McAlinn2017} we label our modeling framework Bayesian Predictive Synthesis (BPS). The sample period is 01:1970-12:2015, monthly.}
\end{justify}
\renewcommand{\arraystretch}{1.2}
\vspace{1em}
{\bf Panel A: \normalfont Sharpe Ratio} \vspace{0.2cm}\\ 		
\resizebox{1.1\textwidth}{!}{\begin{tabular}{lcccccccccccccccc}
\hline
Industry & \multicolumn{10}{c}{Group-Specific Models}                                                                 & HA    & Full & LASSO & Equal Weight & BMA & BPS \\
\cline{2-11}
         & Value	&Profit	 & Capital	& Soundness	 &Solvency	&Liquidity	&Efficiency	&Other	&Aggregate Fin	&Macro  &\\
\hline
Durbl    & 0.006	&0.054	&0.164	&0.187	&0.062	&0.122	&0.187	&0.184	&0.135	&0.012 &0.449 &-0.073	&0.033	&0.183	&0.150	&0.665\\
NoDurbl  & -0.042	&0.244	&0.044	&0.117	&0.145	&0.182	&0.178	&0.239	&0.110	&0.054 &0.420 &0.121	&0.107	&0.196	&0.174	&0.550 \\
Manuf    & 0.025	&0.010	&0.148	&0.061	&0.229	&0.098	&0.142	&0.296	&0.086	&0.030 &0.433 &-0.056	&0.061	&0.220	&0.297	&0.532\\
Energy   & 0.142	&0.054	&0.247	&0.080	&0.250	&0.189	&0.178	&0.111	&0.097	&0.040 &0.394 &0.137	&0.121	&0.268	&0.237	&0.589\\
HiTech   & 0.101	&0.188	&0.284	&0.167	&0.378	&0.234	&0.141	&0.196	&0.247	&0.084 &0.558 &-0.102	&0.107	&0.406	&0.269	&0.689\\
Health   & 0.196	&0.130	&0.134	&0.048	&0.134	&0.313	&0.192	&0.247	&0.235	&0.106 &0.468 &0.131	&0.188	&0.235	&0.241	&0.611\\
Shops    & 0.080	&0.190	&0.291	&0.072	&0.099	&0.232	&0.113	&0.262	&0.189	&0.133 &0.485 &0.076	&0.214	&0.308	&0.105	&0.658\\
Telecomm & 0.069	&0.203	&0.049	&0.242	&0.134	&0.166	&0.198	&0.075	&0.198	&0.115 &0.465 &0.023	&0.148	&0.275	&0.087	&0.688\\
Utils    & -0.003	&0.107	&0.223	&0.105	&0.252	&0.183	&0.212	&0.299	&0.076	&0.103 &0.387 &0.015	&0.074	&0.240	&0.298	&0.627\\
Other    & -0.001	&0.137	&0.251	&0.081	&0.196	&0.112	&0.186	&0.067	&0.112	&0.116 &0.386 &-0.062	&0.048	&0.175	&0.069	&0.549\\
\hline
    \end{tabular}}%
\vspace{1em}

{\bf Panel B: \normalfont Sharpe Ratio (no-short sales)} \vspace{0.2cm}\\ 		
\resizebox{1.1\textwidth}{!}{\begin{tabular}{lcccccccccccccccc}
\hline
Industry & \multicolumn{10}{c}{Group-Specific Models}                                                                 & HA    & Full & LASSO & Equal Weight & BMA & BPS \\
\cline{2-11}
         & Value	&Profit	 & Capital	& Soundness	 &Solvency	&Liquidity	&Efficiency	&Other	&Aggregate Fin	&Macro  &\\
\hline
Durbl    & 0.206	&0.195	&0.580	&0.237	&0.386	&0.305	&0.308	&0.473	&0.351	&0.189 &0.725 &0.072	&0.345	&0.540	&0.529	&0.820\\
NoDurbl  & 0.072	&0.276	&0.266	&0.274	&0.327	&0.284	&0.404	&0.444	&0.164	&0.128 &0.446 &0.189	&0.135	&0.451	&0.314	&0.554\\
Manuf    & 0.225	&0.299	&0.346	&0.271	&0.236	&0.466	&0.407	&0.438	&0.195	&0.195 &0.462 &0.039	&0.115	&0.508	&0.445	&0.594\\
Energy   & 0.209	&0.090	&0.448	&0.109	&0.268	&0.200	&0.195	&0.344	&0.211	&0.318 &0.395 &0.137	&0.130	&0.314	&0.219	&0.592\\
HiTech   & 0.167	&0.175	&0.269	&0.151	&0.379	&0.305	&0.281	&0.454	&0.248	&0.197 &0.604 &-0.068	&0.187	&0.435	&0.264	&0.681\\
Health   & 0.296	&0.165	&0.338	&0.179	&0.409	&0.532	&0.446	&0.496	&0.424	&0.185 &0.517 &0.225	&0.268	&0.494	&0.476	&0.612\\
Shops    & 0.209	&0.239	&0.467	&0.089	&0.278	&0.333	&0.320	&0.368	&0.273	&0.228 &0.523 &0.036	&0.283	&0.441	&0.290	&0.663\\
Telecomm & 0.153	&0.319	&0.387	&0.192	&0.398	&0.517	&0.239	&0.434	&0.322	&0.243 &0.580 &0.081	&0.161	&0.481	&0.363	&0.774\\
Utils    & 0.221	&0.099	&0.334	&0.156	&0.333	&0.242	&0.309	&0.374	&0.246	&0.236 &0.391 &-0.061	&0.105	&0.424	&0.372	&0.631\\
Other    & 0.151	&0.308	&0.306	&0.147	&0.506	&0.532	&0.333	&0.562	&0.295	&0.351 &0.639 &0.071	&0.163	&0.586	&0.563	&0.746\\
\hline
    \end{tabular}}%
\label{Table002}

\end{sidewaystable}%


==> Tables/Table001.tex <==
% Table generated by Excel2LaTeX from sheet 'Regression'
\begin{sidewaystable}[htbp]
\caption{Statistical Comparison of Models Combination Schemes: Stock Returns Predictability}
\vspace{.1in}
\begin{justify}
\footnotesize{This table reports the out-of-sample comparison of our predictive framework against standard model combination methodologies, across ten different industries. Performance comparison is based on the Root Mean Squared Error (RMSE), and the Log Predictive Density Ratio (LPDR) as in Equation \eqref{eq:lpdr}. We report the results obtained for each of the group-specific predictors, the results obtained by simply taking the historical average of the stock returns (HA), and the results from a set of competing model combination/shrinkage schemes, e.g., LASSO, PCA, Equal Weight, and Bayesian Model Averaging (BMA). The sample period is 01:1970-12:2015, monthly.}
\end{justify}
\renewcommand{\arraystretch}{1.2}
\vspace{1em}
{\bf Panel A: \normalfont Root Mean Squared Error} \vspace{0.2cm}\\ 		
\resizebox{1\textwidth}{!}{\begin{tabular}{lcccccccccccccccc}
\hline
Industry & \multicolumn{10}{c}{Group-Specific Models}                                                                 & HA    & LASSO&PCA & Equal Weight & BMA & DRS \\
\cline{2-11}
         & Value	&Profit	 & Capital	& Soundness	 &Solvency	&Liquidity	&Efficiency	&Other	&Aggregate Fin	&Macro  &\\
\hline
Durbl    & 0.102	&0.103	 &0.085	    &0.103	     &0.089	    &0.086	    &0.089	&0.084	&0.086	&0.095  & 0.079  & 0.087&0.091 & 0.084 & 0.081	& 0.078\\
NoDurbl  & 0.044	&0.043	 &0.038	    &0.046	     &0.038	    &0.036	    &0.040	&0.038	&0.041	&0.042  &0.034   &0.045&0.039  & 0.036 & 0.035	&0.034\\
Manuf    & 0.064	&0.072	&0.055	&0.077	&0.057	&0.057	&0.058	&0.054	&0.058	&0.061 &0.052 	&0.055&0.055	&0.054	&0.054	&0.052\\
Energy   & 0.069	&0.086	&0.062	&0.082	&0.064	&0.061	&0.067	&0.061	&0.066	&0.070 & 0.060 	&0.062&0.066	&0.063	&0.061	&0.059\\
HiTech   & 0.078	&0.110	&0.069	&0.105	&0.076	&0.074	&0.079	&0.071	&0.078	&0.083 & 0.069 	&0.073&0.081	&0.071	&0.070	&0.068 \\
Health   & 0.047	&0.052	&0.043	&0.057	&0.042	&0.041	&0.043	&0.041	&0.045	&0.046 & 0.040 	&0.043&0.047	&0.042	&0.041	&0.039\\
Shops    & 0.056	&0.056	&0.047	&0.064	&0.048	&0.047	&0.049	&0.047	&0.051	&0.051 & 0.044 	&0.045&0.063	&0.046	&0.048	&0.043\\
Telecomm & 0.068	&0.064	&0.058	&0.073	&0.058	&0.055	&0.059	&0.058	&0.057	&0.060 & 0.054 	&0.055&0.050	&0.054	&0.058	&0.053\\
Utils    & 0.048	&0.054	&0.043	&0.072	&0.044	&0.045	&0.046	&0.041	&0.047	&0.048 & 0.041 	&0.045&0.060	&0.042	&0.041	&0.040\\
Other    & 0.071	&0.070	&0.056	&0.084	&0.057	&0.057	&0.060	&0.056	&0.063	&0.062 & 0.054 	&0.058&0.046	&0.056	&0.056	&0.053\\
\hline
    \end{tabular}}%
\vspace{1em}

{\bf Panel B: \normalfont Log-Predictive Density Ratio} \vspace{0.2cm}\\ 		
\resizebox{1\textwidth}{!}{\begin{tabular}{lcccccccccccccccc}
\hline
Industry & \multicolumn{10}{c}{Group-Specific Models}                                                                 & HA     & LASSO&PCA & Equal Weight & BMA & DRS \\
\cline{2-11}
         & Value	&Profit	 & Capital	& Soundness	 &Solvency	&Liquidity	&Efficiency	&Other	&Aggregate Fin	&Macro  &\\
\hline
Durbl    & -76.59	&-91.97	&-36.33	&-93.09	  &-44.81	&-39.51	&-45.30	&-34.21	&-44.15	&-62.84 &-23.67  	  &-158.4&-29.38	&-24.06	&-34.69	&-\\
NoDurbl  & -66.96	&-64.74	&-25.99	&-77.46	  &-30.96	&-17.77	&-34.80	&-23.95	&-44.61	&-49.45 &-10.12  	  &-23.47&-38.70	&-15.81	&-18.74	&-\\
Manuf    & -65.68	&-88.08	&-29.68	&-132.12	&-36.36	&-34.08	&-39.40	&-23.94	&-45.47	&-51.13 &-18.62  	  &-57.01&-12.60	&-14.75	&-23.00	& -\\
Energy   & -31.77	&-93.31	&-9.96	&-83.42	  &-14.61	&-5.77	&-24.30	&-6.08	&-19.92	&-32.40 &-2.83   	  &-83.71&-3.46	&-8.93	  &-6.61	  &-\\
HiTech   & -47.46	&-95.81	&-20.39	&-101.32	&-28.36	&-29.41	&-40.36	&-22.14	&-37.87	&-48.17 & -16.10 	&-103.0&-126.73	&-19.34	&-20.92	&-\\
Health   & -43.09	&-77.01	&-20.48	&-90.36	  &-17.71	&-12.62	&-26.84	&-12.33	&-36.88	&-40.45 & -8.09  	&-18.26&-59.94	&-11.04	&-13.67	&-\\
Shops    & -59.31	&-61.68	&-19.50	&-100.51	&-24.30	&-20.11	&-26.68	&-19.07	&-36.97	&-35.68 & -8.49  	&-35.10&-75.45	&-15.92	&-23.90	&-\\
Telecomm & -85.13	&-57.67	&-37.53	&-83.81	  &-37.00	&-30.89	&-43.95	&-32.30	&-38.45	&-48.80 & -22.33 	&-56.72&-2.56	&-23.68	&-31.34	&-\\
Utils    & -43.13	&-66.39	&-15.49	&-146.62	&-19.73	&-24.01	&-28.36	&-12.03	&-39.62	&-44.05 & -10.98 	&-20.50&-126.26	&-11.21	&-12.09	&-\\
Other    & -108.53&-89.30	&-39.48	&-150.83	&-40.52 &-38.49	&-45.34	&-38.71	&-72.47	&-58.40 & -29.26 	&-66.55&-10.01	&-23.81	&-38.57	&-\\
\hline
    \end{tabular}}%
\label{tab:Table001}

\end{sidewaystable}%


==> Tables/Table002.tex <==
% Table generated by Excel2LaTeX from sheet 'Regression'
\begin{sidewaystable}[htbp]
\caption{Economic Comparison of Models Combination Schemes: Stock Returns Predictability}
\vspace{.1in}
\begin{justify}
\footnotesize{This table reports the out-of-sample comparison of our predictive framework against standard model combination methodologies, across ten different industries. Performance comparison is based on the Sharpe Ratio (SR), and its modification whereby short sales are not allowed. We report the results obtained for each of the group-specific predictors, the results obtained by simply taking the historical average of the stock returns (HA), and the results from a set of competing model combination/shrinkage schemes, e.g., LASSO, PCA, Equal Weight, and Bayesian Model Averaging (BMA). The sample period is 01:1970-12:2015, monthly.}
\end{justify}
\renewcommand{\arraystretch}{1.2}
\vspace{1em}
{\bf Panel A: \normalfont Sharpe Ratio} \vspace{0.2cm}\\ 		
\resizebox{1\textwidth}{!}{\begin{tabular}{lcccccccccccccccc}
\hline
Industry & \multicolumn{10}{c}{Group-Specific Models}                                                                 & HA   & LASSO&PCA & EW & BMA & DRS \\
\cline{2-11}
         & Value	&Profit	 & Capital	& Soundness	 &Solvency	&Liquidity	&Efficiency	&Other	&Agg Fin	&Macro  &\\
\hline
Durbl    & 0.006	&0.054	&0.164	&0.187	&0.062	&0.122	&0.187	&0.184	&0.135	&0.012  &0.449	&0.151&0.157	&0.183	&0.150	&0.665\\
NoDurbl  & -0.042	&0.244	&0.044	&0.117	&0.145	&0.182	&0.178	&0.239	&0.110	&0.054  &0.420	&0.058&0.135	&0.196	&0.174	&0.550 \\
Manuf    & 0.025	&0.010	&0.148	&0.061	&0.229	&0.098	&0.142	&0.296	&0.086	&0.030  &0.433	&0.137&0.164	&0.220	&0.297	&0.532\\
Energy   & 0.142	&0.054	&0.247	&0.080	&0.250	&0.189	&0.178	&0.111	&0.097	&0.040  &0.395	&0.168&0.284	&0.268	&0.237	&0.589\\
HiTech   & 0.101	&0.188	&0.284	&0.167	&0.378	&0.234	&0.141	&0.196	&0.247	&0.084  &0.558	&0.305&0.185	&0.406	&0.269	&0.689\\
Health   & 0.196	&0.130	&0.134	&0.048	&0.134	&0.313	&0.192	&0.247	&0.235	&0.106  &0.468	&0.145&0.218	&0.235	&0.241	&0.611\\
Shops    & 0.080	&0.190	&0.291	&0.072	&0.099	&0.232	&0.113	&0.262	&0.189	&0.133  &0.485	&0.169&0.086	&0.308	&0.105	&0.658\\
Telecomm & 0.069	&0.203	&0.049	&0.242	&0.134	&0.166	&0.198	&0.075	&0.198	&0.115  &0.465	&0.304&0.223	&0.275	&0.087	&0.688\\
Utils    & -0.003	&0.107	&0.223	&0.105	&0.252	&0.183	&0.212	&0.299	&0.076	&0.103  &0.387	&0.244&0.215	&0.240	&0.298	&0.627\\
Other    & -0.001	&0.137	&0.251	&0.081	&0.196	&0.112	&0.186	&0.067	&0.112	&0.116  &0.386	&0.081	&0.116 &0.175	&0.069	&0.549\\
\hline
    \end{tabular}}%
\vspace{1em}

{\bf Panel B: \normalfont Sharpe Ratio (no-short sales)} \vspace{0.2cm}\\ 		
\resizebox{1\textwidth}{!}{\begin{tabular}{lcccccccccccccccc}
\hline
Industry & \multicolumn{10}{c}{Group-Specific Models}                                                                 & HA    & LASSO&PCA & EW & BMA & DRS \\
\cline{2-11}
         & Value	&Profit	 & Capital	& Soundness	 &Solvency	&Liquidity	&Efficiency	&Other	&Agg Fin	&Macro  &\\
\hline
Durbl    & 0.206	&0.195	&0.580	&0.237	&0.386	&0.305	&0.308	&0.473	&0.351	&0.189 &0.725 	&0.235&0.530	&0.540	&0.529	&0.820\\
NoDurbl  & 0.072	&0.276	&0.266	&0.274	&0.327	&0.284	&0.404	&0.444	&0.164	&0.128 &0.446 	&0.119&0.339	&0.451	&0.314	&0.554\\
Manuf    & 0.225	&0.299	&0.346	&0.271	&0.236	&0.466	&0.407	&0.438	&0.195	&0.195 &0.462 	&0.139&0.127	&0.508	&0.445	&0.594\\
Energy   & 0.209	&0.090	&0.448	&0.109	&0.268	&0.200	&0.195	&0.344	&0.211	&0.318 &0.395 	&0.243&0.293	&0.314	&0.219	&0.592\\
HiTech   & 0.167	&0.175	&0.269	&0.151	&0.379	&0.305	&0.281	&0.454	&0.248	&0.197 &0.604 	&0.373&0.249	&0.435	&0.264	&0.681\\
Health   & 0.296	&0.165	&0.338	&0.179	&0.409	&0.532	&0.446	&0.496	&0.424	&0.185 &0.517 	&0.265&0.241	&0.494	&0.476	&0.612\\
Shops    & 0.209	&0.239	&0.467	&0.089	&0.278	&0.333	&0.320	&0.368	&0.273	&0.228 &0.523 	&0.241&0.374	&0.441	&0.290	&0.663\\
Telecomm & 0.153	&0.319	&0.387	&0.192	&0.398	&0.517	&0.239	&0.434	&0.322	&0.243 &0.580 	&0.412&0.214	&0.481	&0.363	&0.774\\
Utils    & 0.221	&0.099	&0.334	&0.156	&0.333	&0.242	&0.309	&0.374	&0.246	&0.236 &0.391 	&0.260&0.276	&0.424	&0.372	&0.631\\
Other    & 0.151	&0.308	&0.306	&0.147	&0.506	&0.532	&0.333	&0.562	&0.295	&0.351 &0.639 	&0.152&0.190	&0.586	&0.563	&0.746\\
\hline
    \end{tabular}}%
\label{tab:Table002}

\end{sidewaystable}%

